UniFlow: A Foundation Model for Unified Urban Spatio-Temporal Flow Prediction

Urban spatio-temporal flow prediction, encompassing traffic flows and crowd flows, is crucial for optimizing city infrastructure and managing traffic and emergency responses. Traditional approaches have relied on separate models tailored to either grid-based data, representing cities as uniform cells, or graph-based data, modeling cities as networks of nodes and edges. In this paper, we build UniFlow, a foundational model for general urban flow prediction that unifies both grid-based and graphbased data. We first design a multi-view spatio-temporal patching mechanism to standardize different data into a consistent sequential format and then introduce a spatio-temporal transformer architecture to capture complex correlations and dynamics. To leverage shared spatio-temporal patterns across different data types and facilitate effective cross-learning, we propose SpatioTemporal Memory Retrieval Augmentation (ST-MRA). By creating structured memory modules to store shared spatio-temporal patterns, ST-MRA enhances predictions through adaptive memory retrieval. Extensive experiments demonstrate that UniFlow outperforms existing models in both grid-based and graph-based flow prediction, excelling particularly in scenarios with limited data availability, showcasing its superior performance and broad applicability. The datasets and code implementation have been released on https://github.com/YuanYuan98/UniFlow.

==> 10.bio.tex <==
%\newpage

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.6in,clip,keepaspectratio]{bio_figures/yuanyuan}}]{Yuan Yuan} received the B.S. degree in electronic engineering from Tsinghua University, Beijing, China, in 2020. She is currently working towards the PhD degree with the Department of Electronic Engineering, Tsinghua University (advised by Prof. Yong Li and Prof. Depeng Jin). Her current research interests mainly focus on urban foundation models, urban simulations and generative modeling of spatio-temporal systems. She has publications in conferences and journals such as ICLR, KDD, WWW, and TKDE, etc.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.0in,height=1.5in,clip,keepaspectratio]{bio_figures/ding}}]{Jingtao Ding} received the B.S. degrees in electronic engineering and the Ph.D. degree in electronic engineering from Tsinghua University, Beijing, China, in 2015 and 2020, respectively. He is currently a Post-Doctoral Research Fellow with the Department of Electronic Engineering, Tsinghua University. His research interests include mobile computing, spatiotemporal data mining and user behavior modeling. He has over 30 publications in journals and conferences such as TKDE, TOIS, KDD, NeurIPS, WWW, ICLR, SIGIR, IJCAI, etc.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1.0in,height=1.5in,clip,keepaspectratio]{bio_figures/hch}}]{Chonghua Han} received the B.S. degree from the School of Mechatronical Engineering at Beijing Institute of Technology, Beijing, China, in 2024. He is currently pursuing the M.S. degree in the Department of Electronic Engineering at Tsinghua University. His primary research interests lie in spatio-temporal data mining and deep learning.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1.0in,height=1.4in,clip,keepaspectratio]{bio_figures/jin}}]{Depeng Jin}
 (M'2009) received his B.S. and Ph.D. degrees from Tsinghua University,  Beijing, China, in 1995 and 1999 respectively both in electronics engineering. Now he is an associate professor at Tsinghua University and vice chair of Department of Electronic Engineering. Dr. Jin was
 awarded National Scientific and Technological Innovation Prize  (Second Class) in 2002. His research fields include telecommunications, high-speed networks, ASIC design and future internet architecture.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.0in,height=1.4in,clip,keepaspectratio]{bio_figures/yongli}}]{Yong Li}(M'09-SM'16) received the B.S. degree in electronics and information engineering from Huazhong University of Science and Technology, Wuhan, China, in 2007 and the Ph.D. degree in electronic engineering from Tsinghua University, Beijing, China, in 2012. He is currently a professor of the Department of Electronic Engineering, Tsinghua University.
Prof. Li has served as General Chair, TPC Chair, SPC/TPC Member for several international workshops and conferences, and he is on the editorial board of two IEEE journals. His papers have total citations more than 27000. Among them, ten are ESI Highly Cited Papers in Computer Science, and four receive conference Best Paper (run-up) Awards. He received IEEE 2016 ComSoc Asia-Pacific Outstanding Young Researchers, Young Talent Program of China Association for Science and Technology, and the National Youth Talent Support Program.

\end{IEEEbiography}



==> Algorithm/finetune.tex <==


\algrenewcommand\algorithmicprocedure{\textbf{Step}}
\begin{algorithm}[t]
\caption{Prompt Tuning}\label{alg:finetune}
\begin{algorithmic}[1]

\State \textbf{Input}:  Dataset $D=\{D_1, D_2, \ldots, D_{M}\}$, parameters of pre-trained base model $\theta$, and loss function $L$
\State \textbf{Initialize}: Learnable parameters $\phi$ for the prompt network $G$.
\State Load the pretrained model parameters $\theta$.
\State Fix the parameters of the attention and feed-forward layers of the base model $F_\theta$. 
\For{$epoch\in\{1,2,\ldots,N_{iter}\}$}
    \State Randomly sample a dataset $D_m$ and a mini-batch $(X, Y)$ from $D_m$. 
    \State Generate the prompt $P$  for the mini-batch $P \leftarrow G{\phi}(X)$.
    \State Add the prompt to the input space $X_{p} = X + P$. 
    \State Compute the predictions $\hat{y} \leftarrow F_{\theta}(X_p)$
    \State Compute the MSE loss $\mathcal{L} \leftarrow L(\hat{y},Y)$
    \State Update the model's parameters $\gamma \leftarrow update(\mathcal{L};\gamma), \theta \leftarrow update(\mathcal{L};\theta)$
\EndFor
\end{algorithmic}
\end{algorithm}



==> Tables/few-shot.tex <==
\begin{table*}[t!]
\caption{Performance comparison in few-shot and zero-shot (only UniST)  learning settings on the Crowd dataset in terms of MAE and RMSE. 1\% , 5\%, and 10\% denote that only the percentage of training data is utilized.  We use the average prediction errors over all prediction steps. 
%Bold denotes the best results and \underline{underline} denotes the second-best results.
}\label{tbl:few_shot_crowd}
\begin{threeparttable}
\resizebox{1.5\columnwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
& \multicolumn{2}{c}{\textbf{10\%}} & \multicolumn{2}{c}{\textbf{5\%}} & \multicolumn{2}{c}{\textbf{1\%}}  \\ 
 \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
 \textbf{Model} & \textbf{RMSE}  & \textbf{MAE}    & \textbf{RMSE}    & \textbf{MAE}   & \textbf{RMSE}    & \textbf{MAE}     \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 

ATFM & 19.842 & 11.446  & 19.923 & 11.687 & 21.166 & 12.643 \\
STNorm & 14.668 & 7.050 &  14.884 & 7.723 & 35.959 & 29.585 \\
STID  & 14.676 & 7.280 & 14.975 & 8.671 & 25.905 & 19.610 \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
PredRNN & 19.604 & 9.668 & 20.186 & 10.190 & 24.901 & 13.142 \\
SimVP & 14.093 & 7.101 & 14.167 & 8.550 &  14.252 & 8.776 \\
TAU &14.229 & 7.140 & 14.456 & 8.411 & 14.919 & 9.096  \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
MAML & 14.089 & 7.180 & 14.795 & 8.154 & 14.334 & 8.608\\
MetaST & 13.801 & 6.847 &  14.220 & 7.442 & 14.242& 7.949\\
PatchTST & 14.060 & 6.787  & 14.142 &  6.811 & 14.491 &  7.227 \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
UniST (few-shot)  &13.411 & 6.365 & 13.859 & 6.542 & 13.952 & 6.581  \\
UniST (zero-shot)  & 14.665 & 7.051  & 14.665 & 7.051 & 14.665 & 7.051\\
\bottomrule
\end{tabular}}
\end{threeparttable}
\end{table*}




\begin{table*}[t!]
\caption{Performance comparison in few-shot and zero-shot (only UniST)  learning settings on the BikeNYC dataset in terms of MAE and RMSE. 1\% , 5\%, and 10\% denote that only the percentage of training data is utilized.  We use the average prediction errors over all prediction steps. 
%Bold denotes the best results and \underline{underline} denotes the second-best results.
}\label{tbl:few_shot_bike}
\begin{threeparttable}
\resizebox{1.5\columnwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
& \multicolumn{2}{c}{\textbf{10\%}} & \multicolumn{2}{c}{\textbf{5\%}} & \multicolumn{2}{c}{\textbf{1\%}}  \\ 
 \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
 \textbf{Model} & \textbf{RMSE}  & \textbf{MAE}    & \textbf{RMSE}    & \textbf{MAE}   & \textbf{RMSE}    & \textbf{MAE}     \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 

ATFM & 8.026 & 3.511 & 10.438 &  4.582 &  11.876 & 5.990\\
STNorm & 7.42 & 2.70 & 10.21 & 4.17 & 12.94 & 5.20\\
STID  &  6.97 & 3.49 & 12.46 & 7.56 & 15.08 & 9.38 \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
PredRNN &11.05 & 4.00 & 11.29 & 4.46 & 12.58 & 4.75\\
SimVP &6.570 & 2.691 & 8.525 & 3.174 & 8.661 & 3.721  \\
TAU & 7.06 & 3.07 & 8.74 & 3.28 & 8.50 & 3.72 \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
MAML & 6.49 & 2.31 & 8.89 & 3.68 & 8.98 & 3.91\\ 
MetaST &6.21 & 2.18 & 8.22 & 3.03 & 8.58 & 3.60 \\
PatchTST & 9.14 & 2.68 & 10.09 & 2.88 &  9.74 & 3.86 \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
UniST  & 5.318 & 1.668 & 6.113 & 1.964 & 7.811 & 2.72\\
UniST (zero-shot)  & 9.06 & 3.63 & 9.06 & 3.63 &  9.06 & 3.63 \\
\bottomrule
\end{tabular}}
\end{threeparttable}
\end{table*}


\begin{table*}[t!]
\caption{Performance comparison in few-shot and zero-shot (only UniST) learning settings on the TaxiBJ dataset in terms of MAE and RMSE. 1\% , 5\%, and 10\% denote that only the percentage of training data is utilized.  We use the average prediction errors over all prediction steps. 
%Bold denotes the best results and \underline{underline} denotes the second-best results.
}\label{tbl:few_shot_taxibj}
\begin{threeparttable}
\resizebox{1.5\columnwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
& \multicolumn{2}{c}{\textbf{10\%}} & \multicolumn{2}{c}{\textbf{5\%}} & \multicolumn{2}{c}{\textbf{1\%}}  \\ 
 \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
 \textbf{Model} & \textbf{RMSE}  & \textbf{MAE}    & \textbf{RMSE}    & \textbf{MAE}   & \textbf{RMSE}    & \textbf{MAE}     \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 

ATFM & 50.631 & 33.035 & 55.770 & 39.205 & 64.590 & 44.928 \\
STNorm &39.35 & 22.48 & 42.67 & 26.78 & 44.76 & 28.24 \\
STID  & 34.53 & 20.54 & 37.39 & 24.35 & 47.94 & 31.94 \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
PredRNN & 84.28 & 58.52 & 97.74 & 73.40 & 92.21 & 66.76 \\
SimVP & 35.114 & 20.87 & 37.42 & 23.131 & 40.465 & 24.95 \\
TAU & 37.70 & 22.69 & 39.77 & 25.73 & 41.98 & 26.48 \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
MAML & 36.24 & 20.91 & 36.12 & 23.47 & 40.11 & 24.79 \\ 
MetaST & 35.42 & 18.65 & 35.21 & 21.74 & 39.08 & 23.88\\
PatchTST &  44.03& 22.69 & 44.24 & 22.62 & 46.43 & 24.77  \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
UniST  & 27.59 & 15.18 & 31.19 & 17.58 & 35.09 & 20.62\\
UniST (zero-shot)  & 51.4 & 33.1 &  51.4 & 33.1 & 51.4 & 33.1 \\
\bottomrule
\end{tabular}}
\end{threeparttable}
\end{table*}


==> Tables/model_param.tex <==


\begin{table*}[t!]
\caption{The parameter details of UniST with different sizes evaluated in ablation studies.}\label{tbl:model_info}
\begin{threeparttable}
\resizebox{1.8\columnwidth}{!}{
\begin{tabular}{ccccc}
\toprule
Model & \#Encoder  Layers & \#Decoder Layers & Hidden Dimension (Encoder) & Decoder Hidden Dimension (Decoder)  \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-2}   \cmidrule(lr){3-3}    \cmidrule(lr){4-4}   \cmidrule(lr){5-5}
2M Params  & 2 &  2 &  64  & 64  \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-2}   \cmidrule(lr){3-3}    \cmidrule(lr){4-4}   \cmidrule(lr){5-5}
 8M Params & 4 &3   &  128 & 128   \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-2}   \cmidrule(lr){3-3}    \cmidrule(lr){4-4}     \cmidrule(lr){5-5}
10M Params &  6 & 4 & 128 & 128 \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-2}   \cmidrule(lr){3-3}    \cmidrule(lr){4-4}     \cmidrule(lr){5-5}
15M Params & 8 & 8  & 128 & 128     \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-2}   \cmidrule(lr){3-3}    \cmidrule(lr){4-4}     \cmidrule(lr){5-5}
30M Params & 6 & 6   &  256 & 256    \\ 
\bottomrule
\end{tabular}}
\end{threeparttable}
\end{table*}
